Interpretable Math Word Problem Solution Generation Via Step-by-step Planning

Solutions to math word problems (MWPs) with step-by-step explanations are valuable, especially in education, to help students better comprehend problem-solving strategies. Most existing approaches only focus on obtaining the final correct answer. A few recent approaches leverage intermediate solution steps to improve final answer correctness but often cannot generate coherent steps with a clear solution strategy. Contrary to existing work, we focus on improving the correctness and coherence of the intermediate solutions steps. We propose a step-by-step planning approach for intermediate solution generation, which strategically plans the generation of the next solution step based on the MWP and the previous solution steps. Our approach first plans the next step by predicting the necessary math operation needed to proceed, given history steps, then generates the next step, token-by-token, by prompting a language model with the predicted math operation. Experiments on the GSM8K dataset demonstrate that our approach improves the accuracy and interpretability of the solution on both automatic metrics and human evaluation.

==> 5._Conclusion.tex <==
\section{Conclusions}
In this paper, we addressed the new problem of performing fine-grained, step-by-step controllable solution generation for math word problems. We proposed an approach combining planning and language models to generate interpretable solution steps. Our approach leverages pre-trained language models in two ways: at each step, plan the mathematical operation to be applied, followed by using these plans as prompts to control the token-by-token generation of each step. We demonstrated that with minimal additional parameters introduced, our approach significantly improves math word problem solving performance over simply fine-tuning language models. We also showed that due to the interpretability and high controllability of operation prompts, we can use our approach to generate solutions with alternative strategies by giving it different solution plans. Future work can further explore generating an entire solution path by predicting math operators for each step and revising the plan after each step is generated. We can also explore the application of our approach in real-world educational settings, e.g., for open-ended answer scoring \cite{mlp,edm22}. 


